A new Hybrid Lattice Attack on Galbraith's Binary LWE Cryptosystem

LWE-based cryptosystems are an attractive alternative to traditional ones in the post-quantum era. To minimize the storage cost of part of its public key - a $256 \times 640$ integer matrix, $\textbf{T}$ - a binary version of $\textbf{T}$ has been proposed. One component of its ciphertext, $\textbf{c}_{1}$ is computed as $\textbf{c}_{1} = \textbf{Tu}$ where $\textbf{u}$ is an ephemeral secret. Knowing $\textbf{u}$, the plaintext can be deduced. Given $\textbf{c}_{1}$ and $\textbf{T}$, Galbraith's challenge is to compute $\textbf{u}$ with existing computing resources in 1 year. Our hybrid approach guesses and removes some bits of the solution vector and maps the problem of solving the resulting sub-instance to the Closest Vector Problem in Lattice Theory. The lattice-based approach reduces the number of bits to be guessed while the initial guess based on LP relaxation reduces the number of subsequent guesses to polynomial rather than exponential in the number of guessed bits. Further enhancements partition the set of guessed bits and use a 2-step application of LP. Given the constraint of processor cores and time, a one-time training algorithm learns the optimal combination of partitions yielding a success rate of 9\% - 23\% with 1000 - 100,000 cores in 1 year. This compares favourably with earlier work that yielded 2\% success with 3000 cores.

==> Discussion.tex <==
\section{DISCUSSION}

Limit on success if LP not applied again:
 Following figure represents successful instances when LP is applied only once. A success instance results when different guesses are made and one of the guess results in correcting all wrong bits. Depending upon computation facility more or less number of guess can be done. Correcting each bit needs to make guess of all possible combination as the position of the wrong bit is not known. In the figure \ref{First_Lp}, success of $5.5\%$ can be obtained investing computational time
 
 \begin{align}
   T_{lp} + \sum_{p=1}^{5} \binom{230}{p} \times (T_{LR} + T_{babai})
 \end{align}
 
 Putting proper values for time calculation in above equation results in almost one year with 5,000 cores.   
 
\begin{equation*}
   T_{lp} + \sum_{p=1}^{e_{1}} \binom{i}{p} \Bigg\{ T_{red} + T_{lp} + \sum_{q=1}^{e_{2}} \binom{230-i}{q} \times T_{babai} \Bigg\}
\end{equation*}

Although at first sight it seems calculation time of first approach is less compare to second but its the opposite way around. Its principally because of reduction time. The reduction time of each guess is almost around 3 hours whereas the running time of Babai's algorithm is only 8 second. Considering $5$ errors in $230$ bits needs calculation of almost $356$ days using 5,000 cores whereas breaking it into $2$ errors in $150$ bits and $3$ errors in $80$ bits results in calculation time of 19 days with 5,000 cores, which is a decrease of running time by almost 18 folds.

\paragraph{ 3-way partition }
As a matter of experiment we have thought of 3-way partition and try to calculate the running time to increase the success rate. In 3-way partition time calculation can be done as

\begin{equation*}
    T_{lp} + \sum_{p=1}^{e_{1}} \binom{i}{p} \Bigg\{ T_{lp} + \sum_{q=1}^{e_{2}} \binom{j}{q} \Bigg\{ T_{lp} + T_{LR} + \sum_{r=1}^{e_{3}} \binom{230-i-j}{r} \times T_{babai} \Bigg\} \Bigg\}
\end{equation*}

\paragraph{ Extra strong instances }
% \paragraph{ Comparison with ILP bottom and Middle }

\paragraph{ Implementation of BKZ and Babai's algorithm etc varying block size }

\subsection{\textbf{Choosing proper value for $\alpha$}}
Value of $\alpha$ plays a very important role while solving CVP problem. Therefore, $\alpha$'s value should be chosen properly.
% in such a way that most of the LWE problem can be solved with given number of samples. properly 
% As mentioned earlier we need to find proper value for $q$ to solve $CVP$ problem. 
Laine and Lauter have claimed in \cite{LL} that small error and exponentially large $\alpha$ solves LWE problem with very very high probability. Based on their work, we have performed through experiments considering different values for $\alpha$. Experiments reveals that when prime number of 26 bits is chosen for $\alpha$ then it fetches more than 99 percent success. Increase in $\alpha$ in terms of number of bits results in gradual increase in lattice reduction time while decrease in $\alpha$ value results in decrease reduction time but also reduces the success percent.




==> Introduction_old.tex <==
\begin{abstract}\\
W\\
r\\
i\\
t\\
e\\
a\\
b\\
s\\
t\\
r\\
a\\
c\\
t\\
h\\
e\\
r\\
e\\
\end{abstract}

\keywords{Linear Programming, Learning With Errors, Lattice Reduction, Babai's Algorithm}


 Introduced by Regev  \cite{Regev05} in 2005, Learning with Errors (LWE) is a problem in machine learning and is as hard to solve as certain worst-case lattice problems. Unlike most widely used cryptographic algorithms, it is known to be invulnerable to quantum computers. It is the basis of many cryptographic constructions including 
% Hardness of LWE is the basis of its use in many cryptographic construction including 
IND-CPA and IND-CCA secure encryption \cite{Regev05} \cite{GPV08}, homomorphic encryption \cite{Gentry},  identity-based encryption \cite{CHKP09} \cite{ABB10}, oblivious transfer protocols \cite{PVW08}, lossy-trapdoor functions\cite{PW11}  and many more.

The LWE cryptosystem performs bit by bit encryption. The private key, $\boldsymbol{s}$, is a vector of length $n$ where each element of $\boldsymbol{s}$ is randomly chosen over $\textbf{Z}_q$, $q$ prime. The corresponding public key has two components. The first is a random $m \times n$ matrix, $\boldsymbol{A}$, with elements  over $\textbf{Z}_q$ and with rows denoted $\boldsymbol{a}_i^T$. The second component is a vector, $\boldsymbol{b}$, of length $m$ where the $i^{th}$ element of $\boldsymbol{b}$ is $\boldsymbol{a}_i^T \boldsymbol{s} + e_i$ (mod $q$). The $e_i$'s are drawn from a discretized normal distribution with mean 0 and standard deviation $\sigma$.

To encrypt a bit, $x$, a random binary vector (nonce), $\boldsymbol{u}$,  of length $m$ is chosen. This is a per-message ephemeral secret. The ciphertext is ($\boldsymbol{c}_1$, $c_2$)  where $\boldsymbol{c}_1^T = \boldsymbol{u}^T \boldsymbol{A}$ (mod $q$) and $c_2$ = $\boldsymbol{u}^T \boldsymbol{b} + x \lfloor q/2 \rfloor $ (mod $q$). A received message is  decrypted to 0 or 1 depending on whether $c_2 - \boldsymbol{c}_1 \boldsymbol{s}$ is closer to 0 or $\lfloor q/2 \rfloor$.

 
To thwart various lattice-based attacks, Lindner et al. \cite{lindner2011better} suggested the values of 256, 640 and 4093 respectively for $n$, $m$ and $q$ leading to a public key of size $640 (256 + 1) log_2 (4093) = 246.7$ Kbytes. However, this is far higher than the size of the RSA or ECC public keys which are less than 1 Kbyte.

% This unacceptable storage overhead for resource-constrained devices motivated consideration of binary values in matrix $\boldsymbol{A}$.

% \noindent Regev \cite{Regev05} proposed LWE - a lattice based hard problem. 
To reduce the key size of original LWE problem, the ring LWE cryptosystem was studied in \cite{lyubashevsky2010ideal} and was also shown to be as hard as worst case lattice problems. Another variant of the LWE problem known as Binary-LWE \cite{micciancio2013hardness} was later proposed. Here, the secret is a binary string instead of a string of integers modulo $q$. It results in smaller cryptographic keys without compromising theoretical security guarantees. Hardness of B-LWE problem was proved theoretically in \cite{micciancio2013hardness}. \cite{bai2014lattice} concluded that a key size of 440 is sufficient to make B-LWE as secure as the LWE problem with key size 256. Later another variant of LWE problem, GB-LWE was studied in \cite{galbraith2013space} for devices with low storage capacity. In this case, both the matrix $\boldsymbol{A}$ and secret vector $\boldsymbol{s}$ are binary which further reduces the size of the public key. 

% For $m$ = 640, $n$ = 256 and $q$ = 4093, the LWE crypto scheme provides security equivalent to AES-128 \cite{lindner2011better}. With these parameters, the total size of the public key is $640  (256 + 1)  log_2 (4093) = 246.7$ Kbytes. However, this is far higher than the size of the RSA or ECC public keys which are less than 1 Kbyte. 
In GB-LWE, the binary matrix $\boldsymbol{A}$ is not stored but is generated on the fly using a \textbf{PRNG} %{pseudo random number generator}
with a 256 bit seed \cite{coron2012public}. In this case, we just need to store the seed and the vector $\boldsymbol{b}$, which require $256 + 640 log_2 (4093) = 7935$ bits - a considerable reduction over LWE with non-binary $\boldsymbol{A}$.


% It is the basis of many cryptographic constructions including %IND-CPA and IND-CCA secure encryption \cite{Regev05,gentry2008trapdoors}, 
% identity-based encryption \cite{cash2010bonsai}, \cite{agrawal2010lattice}, oblivious transfer protocols \cite{peikert2008framework}, homomorphic encryption \cite{brakerski2014efficient}, \cite{brakerski2014leveled} %\cite{brakerski2012fully} 
% and many more. %lossy-trapdoor functions\cite{peikert2011lossy}  

% The LWE cryptosystem performs bit by bit encryption. The private key, $\boldsymbol{s}$, is a vector of length $n$ where each element of $\boldsymbol{s}$ is randomly chosen over $\textbf{Z}_q$, $q$ prime. The corresponding public key has two components. The first is a random $m \times n$ matrix, $\boldsymbol{A}$, with elements  over $\textbf{Z}_q$ and with rows denoted $\boldsymbol{a}_i^T$. The second component is a vector, $\boldsymbol{b}$, of length $m$ where the $i^{th}$ element of $\boldsymbol{b}$ is $\boldsymbol{a}_i^T \boldsymbol{s} + e_i$ (mod $q$). The $e_i$'s are drawn from a discretized normal distribution with mean 0 and standard deviation $\sigma$.

% To encrypt a bit, $x$, a random binary vector (nonce), $\boldsymbol{u}$,  of length $m$ is chosen. This is a per-message ephemeral secret. The ciphertext is ($\boldsymbol{c}_1$, $c_2$)  where $\boldsymbol{c}_1^T = \boldsymbol{u}^T \boldsymbol{A}$ (mod $q$) and $c_2$ = $\boldsymbol{u}^T \boldsymbol{b} + x \lfloor q/2 \rfloor $ (mod $q$). A received message is  decrypted to 0 or 1 depending on whether $c_2 - \boldsymbol{c}_1 \boldsymbol{s}$ is closer to 0 or $\lfloor q/2 \rfloor$.




% Recent advances in $quantum$ computers \cite{DS},\cite{JRAAETMBYZ} have triggered widespread interest in development of $post-quantum$ cryptographic schemes\cite{MM}. Traditional number theoretic cryptographic problems such as integer factorization problem and the discrete logarithm problem(both multiplicative groups modulo a prime $p$ and elliptic curve groups) are vulnerable to polynomial time quantum attacks\cite{PZ},\cite{Shor}. The need for $post-quantum$ resistant cryptographic algorithms motivated researchers to explore Lattice cryptography as the same is known to be invulnerable to quantum computers and proved even hard for quantum computers. The field started with seminal work of Ajtai\cite{Ajtai} back in 1996 and recently got a boom after Gentry's breakthrough work \cite{Gentry} on fully homomorphic encryption.

%  One such lattice problem known to be hard for $quantum$ computer is Learning With Error(LWE) problem \cite{Regev05} \cite{Peikert}. LWE, introduced by Regev in \cite{Regev05} is a generalization of Learning Parity With Noise(LPN) problem \cite{KMR94} into large moduli $q$. Hardness of LWE is the basis of its use in many cryptographic construction including IND-CPA and IND-CCA secure encryption \cite{Regev05} \cite{GPV08}, homomorphic encryption \cite{Gentry},  identity-based encryption \cite{CHKP09} \cite{ABB10}, oblivious transfer protocols \cite{PVW08}, lossy-trapdoor functions\cite{PW11}  and many more. 

%  Encryption schemes based on LWE usually performs bit by bit encryption. Private key for encryption is a vector $S$ of size $n$ where each elements are randomly chosen from $\textbf{Z}_q$, $q$ prime. The corresponding public key is a tuple of two components one of them is a matrix $A$ of size $m \times n$, elements are randomly chosen from same field as secret key and the other is $b$, calculated as $b=AS+e \ mod \ q$. The vector $e$ is known as error vector. Elements of the error vectors are drawn from discrete normal distribution with mean $0$ and standard deviation $\sigma$.
 
%  Encryption of a bit x is represented by ciphertext tuple $(c_{1},c_{2})$. First component of the tuple $c_{1}$ is calculated as $\boldsymbol{c}_1^T = \boldsymbol{u}^{T}\boldsymbol{A}$ where $\boldsymbol{u}$ is a random binary vector (nonce) of length $m$. This is a per-message ephemeral secret. Similarly, second component of the touple $c_2$ is obtained as $c_2$ = $\boldsymbol{u}^T \boldsymbol{b} + x \lfloor q/2 \rfloor $ (mod $q$). The received ciphertext tuple $(c_{1},c_{2})$ is decrypted to 0 or 1 depending on whether $c_2 - \boldsymbol{c}_1 \boldsymbol{s}$ is closer to 0 or $\lfloor q/2 \rfloor$.
 
%  Parameter values for $n$, $m$ and $q$  are suggested by linder and peikart in \cite{LL} as 256, 640 and 4093 respectively to thwart  various lattice based attacks. Linder and peikert claimed that above parameters provides security equivalent to AES-128. Setting above values to $n$, $m$ and $q$ leads to public key size of approximately 250 Kbytes, which is unacceptable for resource-constrained devices and motivates researchers to consider binary values in matrix $A$.
 
% To thwart various lattice-based attacks, Lindner et al. \cite{lindner2011better} suggested the values of 256, 640 and 4093 respectively for $n$, $m$ and $q$ leading to a public key of size approximately 250 Kbytes. This unacceptable storage overhead for resource-constrained devices motivated consideration of binary values in matrix $\boldsymbol{A}$.

 
 Galbraith first studied LWE problem considering binary values for matrix $A$ in \cite{SDG13} and also discussed possible attacks on nonce used for encryption to recover the plain-text. He latter posted two challenge, first challenge is to compute $\boldsymbol{u}$ provided random $400 \times 256$ binary matrix $A$ and $\boldsymbol{c_{1}^{T}}$ with $\boldsymbol{c}_1^T = \boldsymbol{u}^{T}\boldsymbol{A}$, within a day using ordinary PC and second challenge is to compute $\boldsymbol{u}$ with matrix $A$ dimension $640 \times 256$ and it should be calculated within a year using "current computing facilities". He further mentioned that breakage of the second challenge will mean total breakage of his paper.
 
 \textbf{Contribution}: The aim of this work is to break Galbraith's second challenge with much higher success percent. Our technique is a unique of its kind. It is a hybrid of Linear Programming (LP) and Lattices. LP is used to pre-process the instance and latter the problem is converted into LWE problem and lattice technique is used to solve the problem.
 
 LP is initially applied on the given instance. Based on the LP output, an initial guess of $x$ bits of the secret are made. A sub-instance is created after removing the $x$ guessed bits. By using a lattice-based approached (rather then ILP \cite{SNDM}) to solve the reduced instance, we require $20\%$ fewer bits to be removed, thus saving computation time by about $300\%$. The problem of obtaining the remaining bits of the secret is mapped to the Closest Vector Problem (CVP) in lattice theory. By using LP, the number of  guessed of the $x$ bits is reduced from exponential to polynomial in $x$. 
 The substantial decrease in execution time is thus due to, both, a fewer number of bits to be guesses and, further, a considerable reduction in the expected number of guesses of the guessed bits.
 
 The second enhancement involves a two-step application of LP. After the first application of LP, $x_1$ bits are guessed and removed. LP is again applied on the reduced sub-instance after which $x_2$ bits are guessed and removed. The lattice-based approach is then employed on the doubly reduced sub-instance. The key advantage of of the two-step approach is that the expected number of errors in the initial guess of $x_1 + x_2=x$ bits is reduced compared to the case of a single application of LP. This translates to a reduction in the number of guesses (and hence execution time) by about $3-4$ orders of magnitude.
 
 For a given $x_1$, $x_2$ and the initial guess of the $x_1 + x_2$ bits, we hypothesize that there are respectively $e_1$ and $e_2$ errors in those bits. Different hypotheses are defined by varying the values of $x_1$, $x_2$, $e_1$, $e_2$. Our strategy is to learn which hypotheses are satisfied by the largest number of the instances while simultaneously factoring the number of guesses (the number of guess is a function of $x_1,x_2,e_1,e_2$). For this purpose, we generate a set of 10,000 random instances and use a variant of the Budgeted Vertex Cover Problem to iteratively select the best hypothesis subject to optimizing an objective function that incorporates the number of new instances added and the execution time. The best hypotheses are then tested with 2,000 random instances. By combining multiple hypotheses, we obtain a substantial improvement in success rate or equivalently a considerable reduction in execution time for a given success rate.
 
%  Our work addresses the second challenge of Galbraith's two challenges. We have found a new technique to solve the galbraith's second challenge and termed it hybrid technique. The idea is to apply Linear programming first and sort the obtained output on the basis of approximate to $.5$ and remove front  $230$ bits.  While removing front bits considered some error in the removed bits and try all combinations to get the correct combinations. For all combinations  convert the reduced sub-instance into LWE problem instance then solve the converted LWE problem. For the correct combination of the front $230$ bits the calculated solution of LWE problem  gives the correct 410 bits and combining the both we can obtain the solution as a whole.
 
%  We have noticed that removing top $230$ in two chunks and applying LP second time increases the success percent. Based on number of bits removed in first step overall success percent varies and results in significant improvement in success percent. Calculating CPU days and corresponding success percent we have provided an algorithm to find the best combinations of bits remove to obtain an approximate optimal success percent. The heuristic provided by us behaves in the same way as training data while testing validating our algorithm.
 
%  We address and solve the second challenge with very high success percent considering affordable CPU days. 
 
\textbf{Notations}: Our convention here is to represent a vector in lowercase bold and a matrix in uppercase bold. A row vector $\boldsymbol{v}$, is represented as $\boldsymbol{v}^T$.
 
\begin{table}[h!] 
% \centering
\begin{tabular}{|p{1.2cm}|p{6.5cm}|}%{ |c|c|c|c|c|c| }
 \hline
 Symbol & Meaning\\
 \hline
 $u_s$ & Sorted and then rounded solution obtained after applying LP once. \\
 \hline
 $x^{'}$ & LP solution sorting on the basis of approximate to $.5$ \\
 \hline
 $u_{s1}$ & First 230 bits of solution \\
 \hline
 $_{2}^{'}$ & Next 256 bits after removing top 230 bits from sorted LP solution \\
 \hline
 $x_{3}^{'}$ & Last 154 bits of sorted LP solution \\
 \hline
 $x_{1,1}^{'}$ & First couple of bits of $x^{'}_{1}$ \\
 \hline
 $x_{1,2}^{'}$ & Next $(x^{'}-x_{1,1}^{'})$/$(230-x_{1,1}^{'})$ bits \\
 \hline
 $i$ & Number of bits removed after applying LP\\
 \hline
 $e_{1}$ & Number of errors in $i$ number of bits.\\
 \hline
 $e_{2}$ & Number of errors in next $(x^{'}-i)$ number of bits.\\
 \hline
 $p(i,e_{1},e_{2})$ & Partition $i$ \\
 \hline
$t_{LP}$ & Computing time of LP \\
\hline
$t_{R}$ & Computing time of lattice reduction \\
\hline
$t_{B}$ & Computing time of Babai's algorithm \\
\hline
\end{tabular}

\caption{Notations}
\label{tab:multipleregimeILP}
\end{table}

